1st Place Solution for YouTubeVOS Challenge 2021:Video Instance Segmentation

Video Instance Segmentation (VIS) is a multi-task problem performing detection, segmentation, and tracking simultaneously. Extended from image set applications, video data additionally induces the temporal information, which, if handled appropriately, is very useful to identify and predict object motions. In this work, we design a unified model to mutually learn these tasks. Specifically, we propose two modules, named Temporally Correlated Instance Segmentation (TCIS) and Bidirectional Tracking (BiTrack), to take the benefit of the temporal correlation between the object's instance masks across adjacent frames. On the other hand, video data is often redundant due to the frame's overlap. Our analysis shows that this problem is particularly severe for the YoutubeVOS-VIS2021 data. Therefore, we propose a Multi-Source Data (MSD) training mechanism to compensate for the data deficiency. By combining these techniques with a bag of tricks, the network performance is significantly boosted compared to the baseline, and outperforms other methods by a considerable margin on the YoutubeVOS-VIS 2019 and 2021 datasets.

==> tex/deeper-pyramid-feature.tex <==
\subsubsection{Deeper pyramid feature}
\label{sec:deeper-pyramid-feature}

FPN \cite{Li2019} is widely adopted to extract features from input image at multiple scales, helping the network to detect objects of different sizes. We started with using 5 levels of feature maps from P2 to P6. After spending more time to analyse object sizes of the dataset, we observe that there are a portion of images having extremely large size(Fig. \ref{fig:scale}), that being said, feature from level P7 is also important to the network, therefore, we end up using features from P2 to P7, ensure that the network is able to fully capture objects of different scales.

\begin{figure}[]
	\centering
	\includegraphics[width=\linewidth]{./images/boxes_scales.png}
	\caption{\small Distribution of width and height of bounding boxes (statistics on rescaled images)} \label{fig:scale}
\end{figure}


==> tex/weight-feat-norm.tex <==
\subsubsection{Weight and Feature Normalization}
\label{sec:weight-feat-norm}

According to the analysis results showing in Fig. \ref{fig:cls_sta}, the imbalance exists in the dataset and is specifically dmoniated by the person class. Usually, the output of classifier predicts the classification logits as  $z = \mathcal{W}^{T} x+b $ where $x$ is the input feature, $\mathcal{W}$ and $b$ is the learnable weights and bias of linear layer respectively. Referring to \cite{norm-cls1, norm-cls2}, the more samples of the training category $i$ the greater $W_i$ will be and it is true for feature $x$. We then visualize the weights of the final classifier in figure \ref{fig:cls_norm}. We achieve figure \ref{fig:cls_norm} as follow. Suppose that the classification weights of shape $W^{C\textrm{x}D}$ with $C$ is the number of classes, $D$ is the feature dimension. The column values in figure \ref{fig:cls_norm} are calculated as:
\begin{equation}
	Val_{colum_i} =  \sqrt{ \sum_{j=1}^D W_{ij}^2 }
\end{equation}
From the abow analysis, we apply normalization on weight and feature to re-balance the scale of weights and features as:
$z=\tau \widetilde{\mathcal{W}}^{T} \widetilde{x}+b$, where $\widetilde{\mathcal{W}}_{i}=\frac{\mathcal{W}_{i}}{\left\|\mathcal{W}_{i}\right\|_{2}}, i \in C, \widetilde{x}=\frac{x}{\|x\|_{2}}$, 
$\tau$ is a temperature factor and set to 20 in our experiments. As a results, the weights of the classifier in figure \ref{fig:cls_norm_w} are less different than  without weight and feature normalization in figure \ref{fig:cls_norm_wo}.

\begin{figure}[]
	\centering
	\includegraphics[width=\linewidth]{"images/cls_sta.png"}
	\caption{\small The classification statistics on YoutubeVOS-VIS training dataset. Class imbalance is presented in the dataset in which the person category is the most common with approximately 35 \%. Roughly 65\% is for 39 other classes.}
	\label{fig:cls_sta}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[b]{\linewidth}
		\includegraphics[width=\linewidth]{images/weight.png}
		\caption{}
		\label{fig:cls_norm_wo} 
	\end{subfigure}

	\begin{subfigure}[b]{\linewidth}
		\includegraphics[width=\linewidth]{images/weight_clsnorm.png}
		\caption{}
		\label{fig:cls_norm_w}
	\end{subfigure}

	\caption{\small The analysis on weight scales of the classifier layer. The weights of classifier layer with (a) and w/o (b) weights and features normalization.}
	\label{fig:cls_norm}
\end{figure}

